Contingency-constrained economic dispatch with safe reinforcement learning

Future power systems will rely heavily on micro grids with a high share of decentralised renewable energy sources and energy storage systems. The high complexity and uncertainty in this context might make conventional power dispatch strategies infeasible. Reinforcement-learning based (RL) controllers can address this challenge, however, cannot themselves provide safety guarantees, preventing their deployment in practice. To overcome this limitation, we propose a formally validated RL controller for economic dispatch. We extend conventional constraints by a time-dependent constraint encoding the islanding contingency. The contingency constraint is computed using set-based backwards reachability analysis and actions of the RL agent are verified through a safety layer. Unsafe actions are projected into the safe action space while leveraging constrained zonotope set representations for computational efficiency. The developed approach is demonstrated on a residential use case using real-world measurements.

==> Safe_RL_for_Economic_Dispatch/graphics/plotstyle.tex <==
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepgfplotslibrary{fillbetween}
\usepackage[nohyperlinks, nolist]{acronym}
\usepackage{amsmath}
\RequirePackage{times}

\pgfplotsset{
	compat=1.16,
	legend image code/.code={ 
		% Set length of legend icon
		\draw[mark repeat=2,mark phase=2]
		plot coordinates {
			(0cm,0cm)
			(0.05cm,0cm)        %% default is (0.3cm,0cm)
			(0.2cm,0cm)         %% default is (0.6cm,0cm)
		};%
	}
}

\definecolorset{RGB}{PLOT}{}{%
	Brown, 153, 79, 0;%
	Black,   0,   0,   0;%
	Blue, 86, 180, 233;%
	DarkBlue, 0, 101, 189;%
	Orange, 230, 159, 0;%
	DarkOrange, 213, 94, 0;%
	Purple, 93, 58, 155;%
	Pink, 220, 38, 127;%
	Red, 227, 27, 35;%
	Yellow, 255, 195, 37;%
	BluishGreen, 0, 158, 115;%
	ReddishPurple, 204, 121, 167;%
	Olive, 162, 173, 0;%
	Gray, 153, 153, 153;%
	Cyan, 64, 176, 166;%
	DarkPurple, 136, 34, 85;%
	TUMBlue, 0, 101, 189;%
	TUMGray, 153, 153, 153;%
	TUMOrange, 227, 114, 34
}

\providecommand{\filepath}{.}
\newcommand{\figpath}{\filepath/data/}

% draws horizontal lines in log scale
\newcommand{\logrewardlines}[0]{
\foreach \i in {4, 3, 2} 
	\foreach \j in {0, 1, ..., 9} 
		\addplot[mark=none, black, samples=2, domain=0:500, line width=0.1pt, color=black!40!white, forget plot]{-log10(\j*10^(\i))};
}
\newcommand{\logrewardlinespenalty}[0]{
\foreach \i in {-1,0,1} 
	\foreach \j in {0, 1, ..., 9} 
		\addplot[mark=none, black, samples=2, domain=0:500, line width=0.1pt, color=black!40!white, forget plot]{log10(\j*10^(\i))};
}
\newcommand{\logrewardlinesday}[0]{
\foreach \i in {-1,0,1} 
	\foreach \j in {0, 1, ..., 9} 
		\addplot[mark=none, black, samples=2, domain=0:1440, line width=0.1pt, color=black!40!white, forget plot]{log10(\j*10^(\i))};
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Plot styles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Logarithmic scale reward plot
% IN:   - Plot commands
%       - Width (6cm)
%       - Height (5cm)
\newcommand{\logrewardplot}[4]{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]
\begin{axis}[width=#2,
    height=#3,
    every tick label/.append style={font=\footnotesize},
    label style={font=\footnotesize},
    ymin=-3.398, ymax=-2,
    xmin=0, xmax=400,
    xtick distance = 100,
    xticklabels={0,0,1,2,3,4},
    ytick={-3,-2},
    yticklabels={-1.000,-100},
    x tick label style={
    	/pgf/number format/.cd,
    	fixed,
    	fixed zerofill,
    	precision=0,
    	/tikz/.cd
    },
    ylabel={Reward},
    xlabel={Steps (in $10^2$)},
	y label style={yshift=-.8em},
	x label style={yshift=.5em},
    legend style={at={(0.99, #4)},anchor=south east,font=\normalfont, nodes={scale=1.0, transform shape}},
    legend cell align={left}
]
\logrewardlines
#1
\end{axis}
\end{tikzpicture}
}

\newcommand{\logpenaltyplot}[4]{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]
\begin{axis}[width=#2,
    height=#3,
    every tick label/.append style={font=\footnotesize},
    label style={font=\footnotesize},
    ymin=-1.3, ymax=1,
    xmin=0, xmax=400,
    xtick distance = 100,
    xticklabels={0,0,1,2,3,4},
    ytick={-1,0,1},
    yticklabels={0.1,1,10},
    x tick label style={
    	/pgf/number format/.cd,
    	fixed,
    	fixed zerofill,
    	precision=0,
    	/tikz/.cd
    },
    ylabel={Penalty},
    xlabel={Steps (in $10^2$)},
	y label style={yshift=-.8em},
	x label style={yshift=.5em},
    legend style={at={(0.99, #4)},anchor=south east,font=\normalfont, nodes={scale=1.0, transform shape}},
    legend cell align={left}
]
\logrewardlinespenalty
#1
\end{axis}
\end{tikzpicture}
}

\newcommand{\logcostplot}[4]{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]
\begin{axis}[width=#2,
    height=#3,
    every tick label/.append style={font=\footnotesize},
    label style={font=\footnotesize},
    ymin=-1.1, ymax=0,
    xmin=0, xmax=400,
    xtick distance = 100,
    xticklabels={0,0,1,2,3,4},
    ytick={-1,0},
    yticklabels={0.1,1},
    x tick label style={
    	/pgf/number format/.cd,
    	fixed,
    	fixed zerofill,
    	precision=0,
    	/tikz/.cd
    },
    ylabel={Cost},
    xlabel={Steps (in $10^2$)},
	y label style={yshift=-.8em},
	x label style={yshift=.5em},
    legend style={at={(0.99, #4)},anchor=south east,font=\normalfont, nodes={scale=1.0, transform shape}},
    legend cell align={left}
]
\logrewardlinespenalty
#1
\end{axis}
\end{tikzpicture}
}

\newcommand{\logsocscsplot}[3]{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]
\begin{axis}[width=#2,
    height=#3,
    every tick label/.append style={font=\footnotesize},
    label style={font=\footnotesize},
    ymin=-0.2, ymax=1,
    xmin=0, xmax=1440,
    xtick={0,240,480,720,960,1200,1440},
    xticklabels={0,4,8,12,16,20,24},
    ytick={0,1},
    yticklabels={1,10},
    x tick label style={
    	/pgf/number format/.cd,
    	fixed,
    	fixed zerofill,
    	precision=0,
    	/tikz/.cd
    },
    ylabel={Sum of Charge States {[kWh]}},
    xlabel={Time {[h]}},
	y label style={yshift=-.8em},
	x label style={yshift=.5em},
    legend style={at={(0.99, 0.7)},anchor=south east,font=\normalfont, nodes={scale=0.8, transform shape}, fill=white, fill opacity=1, draw opacity=1,text opacity=1},
    legend cell align={left}
]
\logrewardlinesday
#1
\end{axis}
\end{tikzpicture}
}

\newcommand{\rewardplot}[4]{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]

\begin{axis}[width=#2,
    height=#3,
    every tick label/.append style={font=\footnotesize},
    label style={font=\footnotesize},
    %axis lines=left,
    %scaled ticks=false,
    ymin=-3000, ymax=0,
    xmin=0, xmax=400,
    xtick distance = 100,
    xticklabels={0,0,1,2,3,4},
    ytick distance = 1000,
    x tick label style={
    	/pgf/number format/.cd,
    	fixed,
    	fixed zerofill,
    	precision=0,
    	/tikz/.cd
    },
    ylabel={Reward},
    xlabel={Steps (in $10^2$)},
    y label style={yshift=-.4em},
    x label style={yshift=.5em},
    legend style={at={(0.99, #4)},anchor=north east,font=\normalfont, nodes={scale=0.7, transform shape}},
    legend cell align={left}
]
{#1}
\end{axis}
\end{tikzpicture}
}

\newcommand{\penaltyplot}[4]{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]

\begin{axis}[width=#2,
    height=#3,
    every tick label/.append style={font=\footnotesize},
    label style={font=\footnotesize},
    %axis lines=left,
    %scaled ticks=false,
    ymin=-0.1, ymax=3.1,
    xmin=0, xmax=400,
    xtick distance = 100,
    xticklabels={0,0,1,2,3,4},
    ytick distance = 1,
    x tick label style={
    	/pgf/number format/.cd,
    	fixed,
    	fixed zerofill,
    	precision=0,
    	/tikz/.cd
    },
    ylabel={Penalty},
    xlabel={Steps (in $10^2$)},
    y label style={yshift=-.4em},
    x label style={yshift=.5em},
    legend style={at={(0.99, #4)},anchor=north east,font=\normalfont, nodes={scale=0.7, transform shape}},
    legend cell align={left}
]
{#1}
\end{axis}
\end{tikzpicture}
}

\newcommand{\costplot}[4]{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]

\begin{axis}[width=#2,
    height=#3,
    every tick label/.append style={font=\footnotesize},
    label style={font=\footnotesize},
    %axis lines=left,
    %scaled ticks=false,
    ymin=-0.05, ymax=1.205,
    xmin=0, xmax=400,
    xtick distance = 100,
    xticklabels={0,0,1,2,3,4},
    ytick distance = 0.2,
    x tick label style={
    	/pgf/number format/.cd,
    	fixed,
    	fixed zerofill,
    	precision=0,
    	/tikz/.cd
    },
    ylabel={Cost},
    xlabel={Steps (in $10^2$)},
    y label style={yshift=-.4em},
    x label style={yshift=.5em},
    legend style={at={(0.99, #4)},anchor=north east,font=\normalfont, nodes={scale=0.7, transform shape}},
    legend cell align={left}
]
{#1}
\end{axis}
\end{tikzpicture}
}

\newcommand{\scsplot}[4]{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]

\begin{axis}[width=#2,
    height=#3,
    every tick label/.append style={font=\footnotesize},
    label style={font=\footnotesize},
    %axis lines=left,
    %scaled ticks=false,
    ymin=-1.05, ymax=1.05,
    xmin=0, xmax=400,
    xtick distance = 100,
    xticklabels={0,0,1,2,3,4},
    ytick distance = 0.2,
    x tick label style={
    	/pgf/number format/.cd,
    	fixed,
    	fixed zerofill,
    	precision=0,
    	/tikz/.cd
    },
    ylabel={Safety Violation},
    xlabel={Steps (in $10^2$)},
    y label style={yshift=-.4em},
    x label style={yshift=.5em},
    legend style={at={(0.99, #4)},anchor=north east,font=\normalfont, nodes={scale=1.0, transform shape}},
    legend cell align={left}
]
{#1}
\end{axis}
\end{tikzpicture}
}

\newcommand{\socvsscsplot}[4]{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]

\begin{axis}[width=#2,
    height=#3,
    every tick label/.append style={font=\footnotesize},
    label style={font=\footnotesize},
    %axis lines=left,
    %scaled ticks=false,
    ymin=0.55, ymax=5.05,
    xmin=0, xmax=1440,
    xtick={0,240,480,720,960,1200,1440},
    xticklabels={0,4,8,12,16,20,24},
    ytick distance = 1,
    x tick label style={
    	/pgf/number format/.cd,
    	fixed,
    	fixed zerofill,
    	precision=0,
    	/tikz/.cd
    },
    ylabel={State of Charge {[kWh]}},
    xlabel={Time {[h]}},
    y label style={yshift=-.4em},
    x label style={yshift=.5em},
    legend style={at={(0.99, #4)},anchor=north east,font=\normalfont, nodes={scale=0.7, transform shape}},
    legend cell align={left}
]
{#1}
\end{axis}
\end{tikzpicture}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Actual plotting commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\plotmeanrewardlog}[2]{


    \pgfplotstablecreatecol[create col/expr={-log10(-min(\thisrow{mean_reward}, -0.00001))}]{log_mean}\data

    \addplot [
    mark=None,
    line width=1pt,
    color=#1,
    solid,
    ] 
    table[
    x = episode,
    y = log_mean,
    ] 
    {\data};
    \addlegendentry{#2}
}
\newcommand{\plotstdrewardlog}[1]{

    %\pgfplotstablecreatecol[create col/expr={-log10(-\thisrow{mean_reward})}]{log_mean}\data
    \pgfplotstablecreatecol[create col/expr={-log10(-min(\thisrow{mean_reward}+\thisrow{std_reward}, -0.00001))}]{log_std_p}\data
    \pgfplotstablecreatecol[create col/expr={-log10(-min(\thisrow{mean_reward}-\thisrow{std_reward}, -0.00001))}]{log_std_m}\data

    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=A,
    ] 
    table[
    x = episode, 
    y = log_std_p,
    ] 
    {\data};
    
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=B,
    ] 
    table[
    x = episode, 
    y = log_std_m,
    ] 
    {\data};
    
    \addplot [
    forget plot,
    color=#1,
    fill opacity=0.2,
    ] 
    fill between [
    of=A and B];
}

\newcommand{\plotmeanreward}[2]{
    \addplot [
    mark=None,
    line width=0.5pt,
    color=#1,
    solid,
    ] 
    table[
    x = episode,
    y = mean_reward
    ] 
    {\data};
    \addlegendentry{#2}
}

\newcommand{\plotstdreward}[1]{
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=A
    ] 
    table[
    x = episode, 
    y expr=(\thisrow{mean_reward}) + \thisrow{std_reward})
    ] 
    {\data};
    
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=B
    ] 
    table[
    x = episode, 
    y expr=(\thisrow{mean_reward}) - \thisrow{std_reward})
    ] 
    {\data};
    
    \addplot [
    forget plot,
    color=#1,
    fill opacity=0.2,
    ] 
    fill between [
    of=A and B];
}

\newcommand{\plotmeanscs}[2]{
    \addplot [
    mark=None,
    line width=0.4pt,
    color=#1,
    solid,
    ] 
    table[
    x = episode,
    y expr= -(\thisrow{mean_scs_violation})
    ] 
    {\data};
    \addlegendentry{#2}
}

\newcommand{\plotminmaxscs}[1]{
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=A,
    ] 
    table[
    x = episode, 
    y expr= -(\thisrow{min_scs_violation})
    ] 
    {\data};
    
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=B,
    ] 
    table[
    x = episode, 
    y expr= -(\thisrow{max_scs_violation})
    ] 
    {\data};
    
    \addplot [
    forget plot,
    color=#1,
    fill opacity=0.2,
    ] 
    fill between [
    of=A and B];
}

\newcommand{\plotmeanpenaltylog}[2]{


    \pgfplotstablecreatecol[create col/expr={log10(\thisrow{mean_penalty})}]{log_mean_penalty}\data

    \addplot [
    mark=None,
    line width=0.5pt,
    color=#1,
    solid,
    ] 
    table[
    x = episode,
    y = log_mean_penalty,
    ] 
    {\data};
    \addlegendentry{#2}
}
\newcommand{\plotstdpenaltylog}[1]{

    %\pgfplotstablecreatecol[create col/expr={-log10(-\thisrow{mean_reward})}]{log_mean}\data
    \pgfplotstablecreatecol[create col/expr={log10(\thisrow{mean_penalty}+\thisrow{std_penalty})}]{log_std_penalty_p}\data
    \pgfplotstablecreatecol[create col/expr={log10(\thisrow{mean_penalty}-\thisrow{std_penalty})}]{log_std_penalty_m}\data

    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=A,
    ] 
    table[
    x = episode, 
    y = log_std_penalty_p,
    ] 
    {\data};
    
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=B,
    ] 
    table[
    x = episode, 
    y = log_std_penalty_m,
    ] 
    {\data};
    
    \addplot [
    forget plot,
    color=#1,
    fill opacity=0.2,
    ] 
    fill between [
    of=A and B];
}

\newcommand{\plotmeanpenalty}[2]{
    \addplot [
    mark=None,
    line width=0.5pt,
    color=#1,
    solid
    ] 
    table[
    x = episode,
    y = mean_penalty
    ] 
    {\data};
    \addlegendentry{#2}
}
\newcommand{\plotstdpenalty}[1]{
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=A
    ] 
    table[
    x = episode, 
    y expr=(\thisrow{mean_penalty}) + \thisrow{std_penalty})
    ] 
    {\data};
    
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=B
    ] 
    table[
    x = episode, 
    y expr=(\thisrow{mean_penalty}) - \thisrow{std_penalty})
    ] 
    {\data};
    
    \addplot [
    forget plot,
    color=#1,
    fill opacity=0.2,
    ] 
    fill between [
    of=A and B];
}

\newcommand{\plotmeancostlog}[2]{


    \pgfplotstablecreatecol[create col/expr={log10(\thisrow{mean_cost})}]{log_mean_cost}\data

    \addplot [
    mark=None,
    line width=0.5pt,
    color=#1,
    solid,
    ] 
    table[
    x = episode,
    y = log_mean_cost,
    ] 
    {\data};
    \addlegendentry{#2}
}
\newcommand{\plotstdcostlog}[1]{

    %\pgfplotstablecreatecol[create col/expr={-log10(-\thisrow{mean_reward})}]{log_mean}\data
    \pgfplotstablecreatecol[create col/expr={log10(\thisrow{mean_cost}+\thisrow{std_cost})}]{log_std_cost_p}\data
    \pgfplotstablecreatecol[create col/expr={log10(\thisrow{mean_cost}-\thisrow{std_cost})}]{log_std_cost_m}\data

    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=A,
    ] 
    table[
    x = episode, 
    y = log_std_cost_p,
    ] 
    {\data};
    
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=B,
    ] 
    table[
    x = episode, 
    y = log_std_cost_m,
    ] 
    {\data};
    
    \addplot [
    forget plot,
    color=#1,
    fill opacity=0.2,
    ] 
    fill between [
    of=A and B];
}

\newcommand{\plotmeancost}[2]{
    \addplot [
    mark=None,
    line width=1pt,
    color=#1,
    solid
    ] 
    table[
    x = episode,
    y = mean_cost
    ] 
    {\data};
    \addlegendentry{#2}
}
\newcommand{\plotstdcost}[1]{
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=A
    ] 
    table[
    x = episode, 
    y expr=(\thisrow{mean_cost}) + \thisrow{std_cost})
    ] 
    {\data};
    
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=B
    ] 
    table[
    x = episode, 
    y expr=(\thisrow{mean_cost}) - \thisrow{std_cost})
    ] 
    {\data};
    
    \addplot [
    forget plot,
    color=#1,
    fill opacity=0.2,
    ] 
    fill between [
    of=A and B];
}

\newcommand{\plotsocscs}[2]{
    \addplot [
    mark=None,
    line width=0.7pt,
    color=#1,
    solid,
    name path=A
    ] 
    table[
    x = time, 
    y = scs_min_sum
    ] 
    {\data};
    \addlegendentry{safe charge state}   
    
    \addplot [
    mark=None,
    line width=0.7pt,
    color=#2,
    dashed,
    name path=B
    ] 
    table[
    x = time, 
    y = soc_sum
    ] 
    {\data};
    \addlegendentry{charge state}
    
    \addplot [
    color=#2,
    fill opacity=0.2,
    ] 
    fill between [
    of=A and B];
}

\newcommand{\plotsocscslog}[2]{
    \pgfplotstablecreatecol[create col/expr={log10(\thisrow{scs_min_sum})}]{log_scs_min_sum}\data
    
    \pgfplotstablecreatecol[create col/expr={log10(\thisrow{soc_sum})}]{log_soc_sum}\data
    
    \addplot [
    mark=None,
    line width=0.7pt,
    color=#1,
    solid,
    name path=A
    ] 
    table[
    x = time, 
    y = log_scs_min_sum
    ] 
    {\data};
    \addlegendentry{safe charge state}   
    
    \addplot [
    mark=None,
    line width=0.7pt,
    color=#2,
    densely dotted,
    name path=B
    ] 
    table[
    x = time, 
    y = log_soc_sum
    ] 
    {\data};
    \addlegendentry{charge state}
    
    \addplot [
    color=#2,
    fill opacity=0.2,
    ] 
    fill between [
    of=A and B];
}

\newcommand{\plotscslog}[1]{
    \pgfplotstablecreatecol[create col/expr={log10(\thisrow{scs_min_sum})}]{log_scs_min_sum}\data
    
    \addplot [
    mark=None,
    forget plot,
    line width=0.7pt,
    color=#1,
    solid,
    name path=A
    ] 
    table[
    x = time, 
    y = log_scs_min_sum
    ] 
    {\data};
    %\addlegendentry{safe charge state}   
        
    \path [forget plot, name path=xaxis]
      (\pgfkeysvalueof{/pgfplots/xmin},\pgfkeysvalueof{/pgfplots/ymin}) --
      (\pgfkeysvalueof{/pgfplots/xmax},\pgfkeysvalueof{/pgfplots/ymin});
    
    \addplot [
    forget plot,
    color=#1,
    fill opacity=0.2,
    ] 
    fill between [
    of=A and xaxis];
    
    \node[text=PLOTTUMOrange, font=\tiny, scale=1.25, fill=white, draw=PLOTTUMOrange, line width=0.7pt] at (650,-0.07) {minimum safe charge state};

}
\newcommand{\plotsoclog}[3]{
    \pgfplotstablecreatecol[create col/expr={log10(\thisrow{soc_sum})}]{log_soc_sum}\data
    
    \addplot [
    mark=None,
    line width=0.7pt,
    color=#1,
    #2,
    name path=A
    ] 
    table[
    x = time, 
    y = log_soc_sum
    ] 
    {\data};
    \addlegendentry{#3}   
}

==> graphics/plotstyle.tex <==
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepgfplotslibrary{fillbetween}
\usepackage[nohyperlinks, nolist]{acronym}
\usepackage{amsmath}
\RequirePackage{times}

\pgfplotsset{
	compat=1.16,
	legend image code/.code={ 
		% Set length of legend icon
		\draw[mark repeat=2,mark phase=2]
		plot coordinates {
			(0cm,0cm)
			(0.05cm,0cm)        %% default is (0.3cm,0cm)
			(0.2cm,0cm)         %% default is (0.6cm,0cm)
		};%
	}
}

\definecolorset{RGB}{PLOT}{}{%
	Brown, 153, 79, 0;%
	Black,   0,   0,   0;%
	Blue, 86, 180, 233;%
	DarkBlue, 0, 101, 189;%
	Orange, 230, 159, 0;%
	DarkOrange, 213, 94, 0;%
	Purple, 93, 58, 155;%
	Pink, 220, 38, 127;%
	Red, 227, 27, 35;%
	Yellow, 255, 195, 37;%
	BluishGreen, 0, 158, 115;%
	ReddishPurple, 204, 121, 167;%
	Olive, 162, 173, 0;%
	Gray, 153, 153, 153;%
	Cyan, 64, 176, 166;%
	DarkPurple, 136, 34, 85;%
	TUMBlue, 0, 101, 189;%
	TUMGray, 153, 153, 153;%
	TUMOrange, 227, 114, 34
}

\providecommand{\filepath}{.}
\newcommand{\figpath}{\filepath/data/}

% draws horizontal lines in log scale
\newcommand{\logrewardlines}[0]{
\foreach \i in {4, 3, 2} 
	\foreach \j in {0, 1, ..., 9} 
		\addplot[mark=none, black, samples=2, domain=0:500, line width=0.1pt, color=black!40!white, forget plot]{-log10(\j*10^(\i))};
}
\newcommand{\logrewardlinespenalty}[0]{
\foreach \i in {-1,0,1} 
	\foreach \j in {0, 1, ..., 9} 
		\addplot[mark=none, black, samples=2, domain=0:500, line width=0.1pt, color=black!40!white, forget plot]{log10(\j*10^(\i))};
}
\newcommand{\logrewardlinesday}[0]{
\foreach \i in {-1,0,1} 
	\foreach \j in {0, 1, ..., 9} 
		\addplot[mark=none, black, samples=2, domain=0:1440, line width=0.1pt, color=black!40!white, forget plot]{log10(\j*10^(\i))};
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Plot styles
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Logarithmic scale reward plot
% IN:   - Plot commands
%       - Width (6cm)
%       - Height (5cm)
\newcommand{\logrewardplot}[4]{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]
\begin{axis}[width=#2,
    height=#3,
    every tick label/.append style={font=\footnotesize},
    label style={font=\footnotesize},
    ymin=-3.398, ymax=-2,
    xmin=0, xmax=400,
    xtick distance = 100,
    xticklabels={0,0,1,2,3,4},
    ytick={-3,-2},
    yticklabels={-1.000,-100},
    x tick label style={
    	/pgf/number format/.cd,
    	fixed,
    	fixed zerofill,
    	precision=0,
    	/tikz/.cd
    },
    ylabel={Reward},
    xlabel={Steps (in $10^2$)},
	y label style={yshift=-.8em},
	x label style={yshift=.5em},
    legend style={at={(0.99, #4)},anchor=south east,font=\normalfont, nodes={scale=1.0, transform shape}},
    legend cell align={left}
]
\logrewardlines
#1
\end{axis}
\end{tikzpicture}
}

\newcommand{\logpenaltyplot}[4]{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]
\begin{axis}[width=#2,
    height=#3,
    every tick label/.append style={font=\footnotesize},
    label style={font=\footnotesize},
    ymin=-1.3, ymax=1,
    xmin=0, xmax=400,
    xtick distance = 100,
    xticklabels={0,0,1,2,3,4},
    ytick={-1,0,1},
    yticklabels={0.1,1,10},
    x tick label style={
    	/pgf/number format/.cd,
    	fixed,
    	fixed zerofill,
    	precision=0,
    	/tikz/.cd
    },
    ylabel={Penalty},
    xlabel={Steps (in $10^2$)},
	y label style={yshift=-.8em},
	x label style={yshift=.5em},
    legend style={at={(0.99, #4)},anchor=south east,font=\normalfont, nodes={scale=1.0, transform shape}},
    legend cell align={left}
]
\logrewardlinespenalty
#1
\end{axis}
\end{tikzpicture}
}

\newcommand{\logcostplot}[4]{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]
\begin{axis}[width=#2,
    height=#3,
    every tick label/.append style={font=\footnotesize},
    label style={font=\footnotesize},
    ymin=-1.1, ymax=0,
    xmin=0, xmax=400,
    xtick distance = 100,
    xticklabels={0,0,1,2,3,4},
    ytick={-1,0},
    yticklabels={0.1,1},
    x tick label style={
    	/pgf/number format/.cd,
    	fixed,
    	fixed zerofill,
    	precision=0,
    	/tikz/.cd
    },
    ylabel={Cost},
    xlabel={Steps (in $10^2$)},
	y label style={yshift=-.8em},
	x label style={yshift=.5em},
    legend style={at={(0.99, #4)},anchor=south east,font=\normalfont, nodes={scale=1.0, transform shape}},
    legend cell align={left}
]
\logrewardlinespenalty
#1
\end{axis}
\end{tikzpicture}
}

\newcommand{\logsocscsplot}[3]{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]
\begin{axis}[width=#2,
    height=#3,
    every tick label/.append style={font=\footnotesize},
    label style={font=\footnotesize},
    ymin=-0.2, ymax=1,
    xmin=0, xmax=1440,
    xtick={0,240,480,720,960,1200,1440},
    xticklabels={0,4,8,12,16,20,24},
    ytick={0,1},
    yticklabels={1,10},
    x tick label style={
    	/pgf/number format/.cd,
    	fixed,
    	fixed zerofill,
    	precision=0,
    	/tikz/.cd
    },
    ylabel={Sum of Charge States {[kWh]}},
    xlabel={Time {[h]}},
	y label style={yshift=-.8em},
	x label style={yshift=.5em},
    legend style={at={(0.99, 0.7)},anchor=south east,font=\normalfont, nodes={scale=0.8, transform shape}, fill=white, fill opacity=1, draw opacity=1,text opacity=1},
    legend cell align={left}
]
\logrewardlinesday
#1
\end{axis}
\end{tikzpicture}
}

\newcommand{\rewardplot}[4]{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]

\begin{axis}[width=#2,
    height=#3,
    every tick label/.append style={font=\footnotesize},
    label style={font=\footnotesize},
    %axis lines=left,
    %scaled ticks=false,
    ymin=-3000, ymax=0,
    xmin=0, xmax=400,
    xtick distance = 100,
    xticklabels={0,0,1,2,3,4},
    ytick distance = 1000,
    x tick label style={
    	/pgf/number format/.cd,
    	fixed,
    	fixed zerofill,
    	precision=0,
    	/tikz/.cd
    },
    ylabel={Reward},
    xlabel={Steps (in $10^2$)},
    y label style={yshift=-.4em},
    x label style={yshift=.5em},
    legend style={at={(0.99, #4)},anchor=north east,font=\normalfont, nodes={scale=0.7, transform shape}},
    legend cell align={left}
]
{#1}
\end{axis}
\end{tikzpicture}
}

\newcommand{\penaltyplot}[4]{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]

\begin{axis}[width=#2,
    height=#3,
    every tick label/.append style={font=\footnotesize},
    label style={font=\footnotesize},
    %axis lines=left,
    %scaled ticks=false,
    ymin=-0.1, ymax=3.1,
    xmin=0, xmax=400,
    xtick distance = 100,
    xticklabels={0,0,1,2,3,4},
    ytick distance = 1,
    x tick label style={
    	/pgf/number format/.cd,
    	fixed,
    	fixed zerofill,
    	precision=0,
    	/tikz/.cd
    },
    ylabel={Penalty},
    xlabel={Steps (in $10^2$)},
    y label style={yshift=-.4em},
    x label style={yshift=.5em},
    legend style={at={(0.99, #4)},anchor=north east,font=\normalfont, nodes={scale=0.7, transform shape}},
    legend cell align={left}
]
{#1}
\end{axis}
\end{tikzpicture}
}

\newcommand{\costplot}[4]{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]

\begin{axis}[width=#2,
    height=#3,
    every tick label/.append style={font=\footnotesize},
    label style={font=\footnotesize},
    %axis lines=left,
    %scaled ticks=false,
    ymin=-0.05, ymax=1.205,
    xmin=0, xmax=400,
    xtick distance = 100,
    xticklabels={0,0,1,2,3,4},
    ytick distance = 0.2,
    x tick label style={
    	/pgf/number format/.cd,
    	fixed,
    	fixed zerofill,
    	precision=0,
    	/tikz/.cd
    },
    ylabel={Cost},
    xlabel={Steps (in $10^2$)},
    y label style={yshift=-.4em},
    x label style={yshift=.5em},
    legend style={at={(0.99, #4)},anchor=north east,font=\normalfont, nodes={scale=0.7, transform shape}},
    legend cell align={left}
]
{#1}
\end{axis}
\end{tikzpicture}
}

\newcommand{\scsplot}[4]{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]

\begin{axis}[width=#2,
    height=#3,
    every tick label/.append style={font=\footnotesize},
    label style={font=\footnotesize},
    %axis lines=left,
    %scaled ticks=false,
    ymin=-1.05, ymax=1.05,
    xmin=0, xmax=400,
    xtick distance = 100,
    xticklabels={0,0,1,2,3,4},
    ytick distance = 0.2,
    x tick label style={
    	/pgf/number format/.cd,
    	fixed,
    	fixed zerofill,
    	precision=0,
    	/tikz/.cd
    },
    ylabel={Safety Violation},
    xlabel={Steps (in $10^2$)},
    y label style={yshift=-.4em},
    x label style={yshift=.5em},
    legend style={at={(0.99, #4)},anchor=north east,font=\normalfont, nodes={scale=1.0, transform shape}},
    legend cell align={left}
]
{#1}
\end{axis}
\end{tikzpicture}
}

\newcommand{\socvsscsplot}[4]{
\begin{tikzpicture}
\tikzstyle{every node}=[font=\footnotesize]

\begin{axis}[width=#2,
    height=#3,
    every tick label/.append style={font=\footnotesize},
    label style={font=\footnotesize},
    %axis lines=left,
    %scaled ticks=false,
    ymin=0.55, ymax=5.05,
    xmin=0, xmax=1440,
    xtick={0,240,480,720,960,1200,1440},
    xticklabels={0,4,8,12,16,20,24},
    ytick distance = 1,
    x tick label style={
    	/pgf/number format/.cd,
    	fixed,
    	fixed zerofill,
    	precision=0,
    	/tikz/.cd
    },
    ylabel={State of Charge {[kWh]}},
    xlabel={Time {[h]}},
    y label style={yshift=-.4em},
    x label style={yshift=.5em},
    legend style={at={(0.99, #4)},anchor=north east,font=\normalfont, nodes={scale=0.7, transform shape}},
    legend cell align={left}
]
{#1}
\end{axis}
\end{tikzpicture}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Actual plotting commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\plotmeanrewardlog}[2]{


    \pgfplotstablecreatecol[create col/expr={-log10(-min(\thisrow{mean_reward}, -0.00001))}]{log_mean}\data

    \addplot [
    mark=None,
    line width=1pt,
    color=#1,
    solid,
    ] 
    table[
    x = episode,
    y = log_mean,
    ] 
    {\data};
    \addlegendentry{#2}
}
\newcommand{\plotstdrewardlog}[1]{

    %\pgfplotstablecreatecol[create col/expr={-log10(-\thisrow{mean_reward})}]{log_mean}\data
    \pgfplotstablecreatecol[create col/expr={-log10(-min(\thisrow{mean_reward}+\thisrow{std_reward}, -0.00001))}]{log_std_p}\data
    \pgfplotstablecreatecol[create col/expr={-log10(-min(\thisrow{mean_reward}-\thisrow{std_reward}, -0.00001))}]{log_std_m}\data

    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=A,
    ] 
    table[
    x = episode, 
    y = log_std_p,
    ] 
    {\data};
    
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=B,
    ] 
    table[
    x = episode, 
    y = log_std_m,
    ] 
    {\data};
    
    \addplot [
    forget plot,
    color=#1,
    fill opacity=0.2,
    ] 
    fill between [
    of=A and B];
}

\newcommand{\plotmeanreward}[2]{
    \addplot [
    mark=None,
    line width=0.5pt,
    color=#1,
    solid,
    ] 
    table[
    x = episode,
    y = mean_reward
    ] 
    {\data};
    \addlegendentry{#2}
}

\newcommand{\plotstdreward}[1]{
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=A
    ] 
    table[
    x = episode, 
    y expr=(\thisrow{mean_reward}) + \thisrow{std_reward})
    ] 
    {\data};
    
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=B
    ] 
    table[
    x = episode, 
    y expr=(\thisrow{mean_reward}) - \thisrow{std_reward})
    ] 
    {\data};
    
    \addplot [
    forget plot,
    color=#1,
    fill opacity=0.2,
    ] 
    fill between [
    of=A and B];
}

\newcommand{\plotmeanscs}[2]{
    \addplot [
    mark=None,
    line width=0.4pt,
    color=#1,
    solid,
    ] 
    table[
    x = episode,
    y expr= -(\thisrow{mean_scs_violation})
    ] 
    {\data};
    \addlegendentry{#2}
}

\newcommand{\plotminmaxscs}[1]{
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=A,
    ] 
    table[
    x = episode, 
    y expr= -(\thisrow{min_scs_violation})
    ] 
    {\data};
    
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=B,
    ] 
    table[
    x = episode, 
    y expr= -(\thisrow{max_scs_violation})
    ] 
    {\data};
    
    \addplot [
    forget plot,
    color=#1,
    fill opacity=0.2,
    ] 
    fill between [
    of=A and B];
}

\newcommand{\plotmeanpenaltylog}[2]{


    \pgfplotstablecreatecol[create col/expr={log10(\thisrow{mean_penalty})}]{log_mean_penalty}\data

    \addplot [
    mark=None,
    line width=0.5pt,
    color=#1,
    solid,
    ] 
    table[
    x = episode,
    y = log_mean_penalty,
    ] 
    {\data};
    \addlegendentry{#2}
}
\newcommand{\plotstdpenaltylog}[1]{

    %\pgfplotstablecreatecol[create col/expr={-log10(-\thisrow{mean_reward})}]{log_mean}\data
    \pgfplotstablecreatecol[create col/expr={log10(\thisrow{mean_penalty}+\thisrow{std_penalty})}]{log_std_penalty_p}\data
    \pgfplotstablecreatecol[create col/expr={log10(\thisrow{mean_penalty}-\thisrow{std_penalty})}]{log_std_penalty_m}\data

    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=A,
    ] 
    table[
    x = episode, 
    y = log_std_penalty_p,
    ] 
    {\data};
    
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=B,
    ] 
    table[
    x = episode, 
    y = log_std_penalty_m,
    ] 
    {\data};
    
    \addplot [
    forget plot,
    color=#1,
    fill opacity=0.2,
    ] 
    fill between [
    of=A and B];
}

\newcommand{\plotmeanpenalty}[2]{
    \addplot [
    mark=None,
    line width=0.5pt,
    color=#1,
    solid
    ] 
    table[
    x = episode,
    y = mean_penalty
    ] 
    {\data};
    \addlegendentry{#2}
}
\newcommand{\plotstdpenalty}[1]{
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=A
    ] 
    table[
    x = episode, 
    y expr=(\thisrow{mean_penalty}) + \thisrow{std_penalty})
    ] 
    {\data};
    
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=B
    ] 
    table[
    x = episode, 
    y expr=(\thisrow{mean_penalty}) - \thisrow{std_penalty})
    ] 
    {\data};
    
    \addplot [
    forget plot,
    color=#1,
    fill opacity=0.2,
    ] 
    fill between [
    of=A and B];
}

\newcommand{\plotmeancostlog}[2]{


    \pgfplotstablecreatecol[create col/expr={log10(\thisrow{mean_cost})}]{log_mean_cost}\data

    \addplot [
    mark=None,
    line width=0.5pt,
    color=#1,
    solid,
    ] 
    table[
    x = episode,
    y = log_mean_cost,
    ] 
    {\data};
    \addlegendentry{#2}
}
\newcommand{\plotstdcostlog}[1]{

    %\pgfplotstablecreatecol[create col/expr={-log10(-\thisrow{mean_reward})}]{log_mean}\data
    \pgfplotstablecreatecol[create col/expr={log10(\thisrow{mean_cost}+\thisrow{std_cost})}]{log_std_cost_p}\data
    \pgfplotstablecreatecol[create col/expr={log10(\thisrow{mean_cost}-\thisrow{std_cost})}]{log_std_cost_m}\data

    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=A,
    ] 
    table[
    x = episode, 
    y = log_std_cost_p,
    ] 
    {\data};
    
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=B,
    ] 
    table[
    x = episode, 
    y = log_std_cost_m,
    ] 
    {\data};
    
    \addplot [
    forget plot,
    color=#1,
    fill opacity=0.2,
    ] 
    fill between [
    of=A and B];
}

\newcommand{\plotmeancost}[2]{
    \addplot [
    mark=None,
    line width=1pt,
    color=#1,
    solid
    ] 
    table[
    x = episode,
    y = mean_cost
    ] 
    {\data};
    \addlegendentry{#2}
}
\newcommand{\plotstdcost}[1]{
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=A
    ] 
    table[
    x = episode, 
    y expr=(\thisrow{mean_cost}) + \thisrow{std_cost})
    ] 
    {\data};
    
    \addplot [
    mark=None,
    forget plot,
    line width=0pt,
    opacity=0,
    name path=B
    ] 
    table[
    x = episode, 
    y expr=(\thisrow{mean_cost}) - \thisrow{std_cost})
    ] 
    {\data};
    
    \addplot [
    forget plot,
    color=#1,
    fill opacity=0.2,
    ] 
    fill between [
    of=A and B];
}

\newcommand{\plotsocscs}[2]{
    \addplot [
    mark=None,
    line width=0.7pt,
    color=#1,
    solid,
    name path=A
    ] 
    table[
    x = time, 
    y = scs_min_sum
    ] 
    {\data};
    \addlegendentry{safe charge state}   
    
    \addplot [
    mark=None,
    line width=0.7pt,
    color=#2,
    dashed,
    name path=B
    ] 
    table[
    x = time, 
    y = soc_sum
    ] 
    {\data};
    \addlegendentry{charge state}
    
    \addplot [
    color=#2,
    fill opacity=0.2,
    ] 
    fill between [
    of=A and B];
}

\newcommand{\plotsocscslog}[2]{
    \pgfplotstablecreatecol[create col/expr={log10(\thisrow{scs_min_sum})}]{log_scs_min_sum}\data
    
    \pgfplotstablecreatecol[create col/expr={log10(\thisrow{soc_sum})}]{log_soc_sum}\data
    
    \addplot [
    mark=None,
    line width=0.7pt,
    color=#1,
    solid,
    name path=A
    ] 
    table[
    x = time, 
    y = log_scs_min_sum
    ] 
    {\data};
    \addlegendentry{safe charge state}   
    
    \addplot [
    mark=None,
    line width=0.7pt,
    color=#2,
    densely dotted,
    name path=B
    ] 
    table[
    x = time, 
    y = log_soc_sum
    ] 
    {\data};
    \addlegendentry{charge state}
    
    \addplot [
    color=#2,
    fill opacity=0.2,
    ] 
    fill between [
    of=A and B];
}

\newcommand{\plotscslog}[1]{
    \pgfplotstablecreatecol[create col/expr={log10(\thisrow{scs_min_sum})}]{log_scs_min_sum}\data
    
    \addplot [
    mark=None,
    forget plot,
    line width=0.7pt,
    color=#1,
    solid,
    name path=A
    ] 
    table[
    x = time, 
    y = log_scs_min_sum
    ] 
    {\data};
    %\addlegendentry{safe charge state}   
        
    \path [forget plot, name path=xaxis]
      (\pgfkeysvalueof{/pgfplots/xmin},\pgfkeysvalueof{/pgfplots/ymin}) --
      (\pgfkeysvalueof{/pgfplots/xmax},\pgfkeysvalueof{/pgfplots/ymin});
    
    \addplot [
    forget plot,
    color=#1,
    fill opacity=0.2,
    ] 
    fill between [
    of=A and xaxis];
    
    \node[text=PLOTTUMOrange, font=\tiny, scale=1.25, fill=white, draw=PLOTTUMOrange, line width=0.7pt] at (650,-0.07) {minimum safe charge state};

}
\newcommand{\plotsoclog}[3]{
    \pgfplotstablecreatecol[create col/expr={log10(\thisrow{soc_sum})}]{log_soc_sum}\data
    
    \addplot [
    mark=None,
    line width=0.7pt,
    color=#1,
    #2,
    name path=A
    ] 
    table[
    x = time, 
    y = log_soc_sum
    ] 
    {\data};
    \addlegendentry{#3}   
}
